Towards Unbiased Evaluation of Detecting Unanswerable Questions in EHRSQL

Incorporating unanswerable questions into EHR QA systems is crucial for testing the trustworthiness of a system, as providing non-existent responses can mislead doctors in their diagnoses. The EHRSQL dataset stands out as a promising benchmark because it is the only dataset that incorporates unanswerable questions in the EHR QA system alongside practical questions. However, in this work, we identify a data bias in these unanswerable questions; they can often be discerned simply by filtering with specific N-gram patterns. Such biases jeopardize the authenticity and reliability of QA system evaluations. To tackle this problem, we propose a simple debiasing method of adjusting the split between the validation and test sets to neutralize the undue influence of N-gram filtering. By experimenting on the MIMIC-III dataset, we demonstrate both the existing data bias in EHRSQL and the effectiveness of our data split strategy in mitigating this bias.

==> tables/new_split_bias.tex <==
\begin{table}[t]
\centering
{\small
\renewcommand{\arraystretch}{1.0}
\resizebox{1.00\columnwidth}{!}{
\begin{tabular}{clclc}
\toprule[1pt]
\multirow{2}{*}{\textbf{Rank}} & \multicolumn{2}{c}{Valid} & \multicolumn{2}{c}{Test} \\
   & Pattern  & ratio & Pattern & ratio \\
\midrule
\Circle \ {\texttt{\,Unigram}} & & & & \\ 
(1) & dr & 19 & department & 35 \\
(2) & outpatient & 19 & effect & 20 \\
(3) & schedule & 19 & appointment & 18 \\
\midrule
\Circle \ {\texttt{\,Bigram}} & & & & \\ 
(1) & outpatient schedule & 18 & other department & 19 \\
(2) & a headache & 13 & side effects & 18 \\
(3) & when does & 13 & blood transfusion & 14 \\
\midrule
\Circle \ {\texttt{\,Trigram}} & & & & \\ 
(1) & when does patient & 12 & the other department & 14 \\
(2) & relieve a headache & 12 & a blood transfusion & 13 \\
(3) & to relieve a & 11 & number of patient & 12 \\
\bottomrule[1pt]
\end{tabular}
}
}
\caption{N-grams have different ratios on new split of validation and test data. }
\label{table:new_split_bias}
\end{table}
